A novel experimental system for the KDK measurement of the $^{40}$K decay scheme relevant for rare event searches

Potassium-40 ($^{40}$K) is a long-lived, naturally occurring radioactive isotope. The decay products are prominent backgrounds for many rare event searches, including those involving NaI-based scintillators. $^{40}$K also plays a role in geochronological dating techniques. The branching ratio of the electron capture directly to the ground state of argon-40 has never been measured, which can cause difficulty in interpreting certain results or can lead to lack of precision depending on the field and analysis technique. The KDK (Potassium (K) Decay (DK)) collaboration is measuring this decay. A composite method has a silicon drift detector with an enriched, thermally deposited $^{40}$K source inside the Modular Total Absorption Spectrometer. This setup has been characterized in terms of energy calibration, gamma tagging efficiency, live time and false negatives and positives. A complementary, homogeneous, method is also discussed; it employs a KSr$_2$I$_5$:Eu scintillator as source and detector.

==> Subfiles/Extra_Parts.tex <==
\section{Extra Parts \label{App:Extra Parts}(Not For Publications)}

Here lies the data not deemed worthy of the paper.

\begin{table}[t]
\centering
 \begin{tabular}{|c|c|} 
    
\hline        
 Component & Voltage (V) \\ \hline
  First \pplus~ring & -10.0  \\ 
 Guard Ring & -20.0 \\
 Amplifier Negative Power & -6.0  \\
 Amplifier Positive Power &  6.0  \\
 Drain of the Integrated FET & 9.65 \\
 Back (\pplus) Contact & -100.0 \\
 Back Contact Protection Ring  & -110.0 \\
 Final Cathode Ring & -150.0  \\
 Guard of Integrated FET & -4.23 \\ 
 Source of Integrated FET & -9.65 \\ 
 Temperature Diode Guard & -10.0\\
 Thermoelectric Cooler Positive Power Supply & 1.77 \\ 
 Thermoelectric Cooler Negative Power Supply & -1.77 \\ \hline
 
 
\end{tabular}
\caption{SDD Operating Parameters}
\label{tab:SDD_Operating_Parameters}
\end{table}




\begin{table}[ht]
\centering
\begin{tabular}{|c|c|} 
\hline        
Coincidence Window ($\mu s$) & Rate (counts/s)  \\\hline
0.1 & 2441.74 $\pm$ 0.15\\
0.2 & 2347.26 $\pm$ 0.14\\
0.3 & 2332.99 $\pm$ 0.14\\
0.5 & 2323.25 $\pm$ 0.14 \\
0.75 & 2318.53 $\pm$ 0.14 \\
1.0 & 2315.21 $\pm$ 0.14 \\
2.0 & 2301.21 $\pm$ 0.14 \\
4.0 & 2278.31 $\pm$ 0.14 \\\hline



\end{tabular}
\caption{Background rate in the MTAS detector as a function of coincidence window. Only events from 0 -1460~keV are considered.}
\label{tab:App_MTAS_BKG_Rate}
\end{table}




\begin{figure}[ht]
  \centering
  \includegraphics[width=0.9\textwidth]{Figures/SDD_Cooling_Loop_Close.pdf}
	\caption{\label{Fig:SDD_Cooling_Loop_Close.pdf}SDD cooling assembly rendering. Cables and screws are not shown.}
\end{figure}
%
%
\begin{figure}[ht]
  \centering
  \includegraphics[width=1.0\textwidth]{Figures/SDD_Vacuum_Chamber_Shielded.png}
\caption{\label{Fig:SDD_Vacuum_Chamber_Shielded.png} Cross-section of the MTAS insert. The SDD cooling setup is visible inside.}

\end{figure}

\begin{table}[ht]
\centering
\begin{tabular}{|c|c|c|}
\hline
Nominal Coincidence Window ($\mu s$) & $^{65}$Zn \BMTAS$T$ & $^{54}$Mn \BMTAS$T$  \\\hline
0.1  & N/A  & 0.0018 $\pm$ 0.0001\\
0.2  & 0.0028 $\pm$ 0.0001 & 0.0028 $\pm$ 0.0001  \\
0.3  & 0.0038 $\pm$ 0.0001 & 0.0036 $\pm$ 0.0001 \\
0.5  & 0.0047 $\pm$ 0.0001 & 0.0046 $\pm$ 0.0001\\
0.75 & 0.0058 $\pm$ 0.0001 & 0.0058 $\pm$ 0.0001\\
1.0  & 0.0070 $\pm$ 0.0001 & 0.0071 $\pm$ 0.0001\\
2.0  & 0.0122 $\pm$ 0.0001 & 0.0122 $\pm$ 0.0001\\
4.0  & 0.0227 $\pm$ 0.0002 & 0.0227 $\pm$ 0.0001\\\hline

\end{tabular}
\caption[]{\label{tab:Beta_T_Tab_App} Measured  \BMTAS$T$ values for the different sources as a function of coincidence windows. Due to low statistics the 0.1~$\mu s$ coincidence window the fit could not be performed. }
\end{table}




==> Subfiles/M54_Efficiency_Model.tex <==


\section{\textcolor{red}{REMOVE THIS, AND ALL THAT FOLLOWS, FOR PUBLICATION}}


\section{\texorpdfstring{\Mn~Efficiency Model}{Mn54 Efficiency Model} (Not For Publication) \label{App:Mn54_Efficiency_Model}}

The gamma tagging efficiency ($\varepsilon_\gamma$) is defined as the probability that MTAS will detect the gamma when triggered by the X-ray (or Auger) in the SDD. \Mn~is an ideal source to study this parameter because it decays almost exclusively through the excited state, giving a $\rho$ (expected ratio of EC~to \ECStar~events) that is very small: $\rho= 3.0 \times 10^{-6}$. This value and the decay scheme of \Mn~are acquired from~\cite{be_table_2004}. The small (almost non-existant) ground state electron capture implies that there should be no false negatives, (where an EC event looks like a \ECStar) during the exposure. In addition, as there should be very few EC events due to the decay scheme of \Mn, the dominant source of events in the anti-coincidence spectrum would be from  \ECStar\ decays whose gamma has not been tagged (i.e. a false positive).
  

\subsection{Anti-coincidence spectrum}

The anti-coincidence spectrum for the \Mn~source is modelled using Eq.~\ref{Eqn:Anti_Fit} for the 5.0--7.0~keV region. Here $C(E)$ is the distribution of events of the anti-coincidence spectrum as a function of energy $E$. It consists of 4 components: $X_{S}$ is the X-ray signal component, $A_{S}$ is the Auger component, $F_{Cont}$ is the $^{55}$Fe contamination,  and $An_{BKG}$ is the flat background contribution. 

The $\Sigma$ term represents the expected anti-coincident X-ray counts and is derived in Lilianna's document: \emph{Effect of SDD Tagging-Efficiency of Conversion Electrons in KDK Analysis}. The $\Sigma$ parameter takes into account the possibility of additional X-rays being produced during an internal conversion. The $\varepsilon_\gamma^\prime$ contains the corrections to the likelihood to include cases where the gamma is missed but the X-ray/Auger arrives in coincidence with a background event in MTAS, shown in Eqn.~\ref{Eqn:epsilon_prime}.


The $\delta$ is a parameters that gives the Augers signal events as a fraction of the total X-ray signal events. From Table~\ref{tab:Par_Val} we see that there are approximately 18000 total Auger events, with almost 99$\%$ being in the coincident window. The probability of internal conversion occurring in \Mn\ is 0.0275$\%$ (see Table~\ref{tab:mn54_ICC}), which would imply that $\sim$5 of the Auger electron capture events, transition through internal conversion. For this reason the effect of conversion electrons is negligible for the Augers. The difference in the measured $\varepsilon_\gamma$ when including the Augers in the signal likelihood can be seen in Table~\ref{tab:W_WO_Auger}.  The definition for the parameters found in Equations~\ref{Eqn:Xray_Signal},~\ref{Eqn:Sigma},~\ref{Eqn:Fe55_Contamination},~\ref{Eqn:Auger_Signal} and~\ref{Eqn:Anti_BKG} are given in Table~\ref{tab:Par_Def}.



%

\begin{equation}\label{Eqn:Anti_Fit} 
C(E) = \underbrace{X_{S}(E)}_\text{X-rays} + \underbrace{A_{S}(E)}_\text{Augers} + \underbrace{F_{Cont}(E)}_\text{Fe \ contamination} + \underbrace{An_{BKG}(E)}_\text{Other \ BGs},
\end{equation}

%
where, 

\begin{equation}\label{Eqn:Xray_Signal} 
X_{S}(E) = \overbrace{\Sigma}^{Expected\ Anti.\ X-ray\ counts}  \ \underbrace{ \frac{1}{R_{Mn}+1}   \left[ \overbrace{ R_{Mn}}^{Ratio \ Ka/Kb} \overbrace{ \frac{1}{\sqrt{2\pi}\sigma_{1}}  e^{-\frac{1}{2}(\frac{E-\mu_{1}}{\sigma_{1}})^2} }^{Ka \ pdf}+   \overbrace{ \frac{1}{\sqrt{2\pi}\sigma_{2}  }  e^{-\frac{1}{2}(\frac{E-\mu_{2}}{\sigma_{2}})^2}}^{Kb \ pdf } \right]}_\text{Ka \ Kb \ pdf},
\end{equation}

%

\begin{equation}\label{Eqn:Sigma}
\Sigma =\underbrace{ \overbrace{\nu}^\text{Expected Total X-Rays} 
    \left[ \frac{\overbrace{ 1 - \varepsilon^\prime_\gamma }^\text{ From Missed $\gamma$}
                +\overbrace{ \alpha_T(1 - \varepsilon_e)
                + \alpha_K(1 - \varepsilon_{e})
                \left(
                    \frac{1}{P_K} - 2\omega_K\eta_E 
                \right)}^\text{From Missed C.E.} }{1+   \alpha_T+\alpha_K  \left( \frac{1}{P_K} - 2\omega_K\eta_E \right)  }\right]}_\text{Expected Anti. X-rays Counts}
\end{equation}




\begin{equation}\label{Eqn:epsilon_prime}
    \varepsilon_\gamma^\prime = \overbrace{\varepsilon_\gamma (1-B_m T)}^\text{see source $\gamma$, miss BKG event} + \overbrace{(1-\varepsilon_\gamma) B_m T}^\text{miss source $\gamma$, see BKG event} + \overbrace{\varepsilon_\gamma B_m T}^\text{See source $\gamma$, see BKG event } + \overbrace{2 A I_{EC*} T \varepsilon_\gamma^2 \eta_E (1-\eta_E) (1-B_M T)}^\text{See two $\gamma$, miss BKG, miss one x-ray}
\end{equation}




\begin{equation}\label{Eqn:Auger_Signal} 
A_{S}(E) = \overbrace{ \delta \nu (1-\varepsilon^\prime_\gamma)}^\text{Expected Anti. Auger Counts} \underbrace{\frac{1}{\sqrt{2\pi}\sigma_{Aug}}  e^{-\frac{1}{2}(\frac{E-\mu_{Aug}}{\sigma_{Aug}})^2}}_\text{Auger\ pdf}
\end{equation}



\begin{equation}\label{Eqn:Fe55_Contamination} 
F_{Cont}(E) = \overbrace{Fe_{Cont}}^\text{Expected \Fe\ counts} \ \underbrace{ \frac{1}{R_{Fe}+1}   \left[ \overbrace{ R_{Fe}}^{Ratio \ Ka/Kb} \overbrace{ \frac{1}{\sqrt{2\pi}\sigma_{3}}  e^{-\frac{1}{2}(\frac{E-\mu_{3}}{\sigma_{3}})^2} }^{Ka \ pdf}+   \overbrace{ \frac{1}{\sqrt{2\pi}\sigma_{3}  }  e^{-\frac{1}{2}(\frac{E-\mu_{4}}{\sigma_{3}})^2}}^{Kb \ pdf } \right]}_\text{Ka \ Kb \ pdf},
\end{equation}





\begin{equation}\label{Eqn:Anti_BKG} 
An_{BKG}(E) = \overbrace{A_{BKG}}^\text{Flat Background}
\end{equation}



\subsection{Coincidence spectrum}

The coincidence spectrum for the \Mn~source is modelled using Eq.~\ref{Eqn:Coinc_Fit} for the 5.0-7.0~keV region. Here Cd(E) is the distribution of events of the coincidence spectrum. It consists of 3 components: $CX_{S}$ is the X-ray signal component, $CA_{S}$ is the Auger component and $Cn_{BKG}$ is a flat the background contribution. 

The $\Sigma^*$  represents the expected coincident X-ray counts and is derived in Liliannas document: \emph{Effect of SDD Tagging-Efficiency of Conversion Electrons in KDK Analysis: Sec. 3.6}. The $\Sigma^*$ parameter takes into account the possibility of additional X-rays being produced during an internal conversion. The $\varepsilon_\gamma^\prime$ contains the corrections to the likelihood to include cases where the gamma is missed but the X-ray/Auger arrives in coincidence with a background event in MTAS, shown in Eqn.~\ref{Eqn:epsilon_prime_2}. The $\delta$ is a parameters that gives the Augers signal events as a fraction of the total X-ray signal events. The definition for the parameters found in Equations~\ref{Eqn:Coinc_Xray_Signal},~\ref{Eqn:Sigma_Star},~\ref{Eqn:Coinc_Auger_Signal} and~\ref{Eqn:Coinc_BKG} are given in Table~\ref{tab:Par_Def}.

\begin{equation}\label{Eqn:Coinc_Fit} 
Cd(E) = \underbrace{CX_{S}(E)}_\text{X-rays} + \underbrace{CA_{S}(E)}_\text{Augers} + \underbrace{Cn_{BKG}(E)}_\text{Other \ BGs},
\end{equation}



where, 

\begin{equation}\label{Eqn:Coinc_Xray_Signal} 
CX_{S}(x) = \overbrace{\Sigma^*}^{Expected\ Coinc.\ X-ray\ counts}  \ \underbrace{ \frac{1}{R_{Mn}+1}   \left[ \overbrace{ R_{Mn}}^{Ratio \ Ka/Kb} \overbrace{ \frac{1}{\sqrt{2\pi}\sigma_{1}}  e^{-\frac{1}{2}(\frac{E-\mu_{1}}{\sigma_{1}})^2} }^{Ka \ pdf}+   \overbrace{ \frac{1}{\sqrt{2\pi}\sigma_{2}  }  e^{-\frac{1}{2}(\frac{E-\mu_{2}}{\sigma_{2}})^2}}^{Kb \ pdf } \right]}_\text{Ka \ Kb \ pdf},
\end{equation}




\begin{equation}\label{Eqn:Sigma_Star}
\Sigma^* =\underbrace{ \overbrace{\nu}^\text{Expected Total X-Rays} 
    \left[ \frac{\overbrace{ \varepsilon^\prime_\gamma }^\text{ From Detected $\gamma$}
                +\overbrace{ \alpha_T \varepsilon_e
                + \alpha_K\varepsilon_{e}
                \left(
                    \frac{1}{P_K} - 2\omega_K\eta_E 
                \right)}^\text{From Detected C.E.} }{1+   \alpha_T+\alpha_K  \left( \frac{1}{P_K} - 2\omega_K\eta_E \right)  }\right]}_\text{Expected Coinc. X-rays counts}
\end{equation}



\begin{equation}\label{Eqn:epsilon_prime_2}
    \varepsilon_\gamma^\prime = \overbrace{\varepsilon_\gamma (1-B_m T)}^\text{see source $\gamma$, miss BKG event} + \overbrace{(1-\varepsilon_\gamma) B_m T}^\text{miss source $\gamma$, see BKG event} + \overbrace{\varepsilon_\gamma B_m T}^\text{See source $\gamma$, see BKG event } + \overbrace{2 A I_{EC*} T \varepsilon_\gamma^2 \eta_E (1-\eta_E) (1-B_M T)}^\text{See two $\gamma$, miss BKG, miss one x-ray}
\end{equation}





\begin{equation}\label{Eqn:Coinc_Auger_Signal} 
CA_{S}(E) =\overbrace{ \delta \nu (\varepsilon^\prime_\gamma)}^\text{Expected Coinc. Auger counts}\underbrace{\frac{1}{\sqrt{2\pi}\sigma_{Aug}}  e^{-\frac{1}{2}(\frac{E-\mu_{Aug}}{\sigma_{Aug}})^2}}_\text{Auger\ pdf},
\end{equation}







\begin{equation}\label{Eqn:Coinc_BKG} 
Cn_{BKG}(E) = \overbrace{C_{BKG}}^\text{Flat Background}.
\end{equation}




\begin{table*}[ht]
\centering
\begin{tabular}{cl}
\hline
Parameter & Definition  \\\hline
E & Energy (keV)\\
$\nu$ & Total number of X-ray signal events (counts)  \\
$\varepsilon_{\gamma}$ & Efficiency of detecting the 835 keV gamma \\
$\mu_{1}$ & Mean Energy of $^{54}$Mn K$_{\alpha}$ X-ray, fixed parameter (5.411~keV) \\
$\sigma_{1}$ & Width of the $^{54}$Mn K$_{\alpha}$ peak (keV)  \\
$\mu_{2}$ & Mean Energy of $^{54}$Mn K$_{\beta}$ X-ray, fixed parameter (5.966~keV) \\
$\sigma_{2}$ & Width of the $^{54}$Mn K$_{\beta}$ peak (keV)  \\
R$_{Mn}$ & Ratio of K$_{\alpha}$ to K$_{\beta}$ for $^{54}$Mn, fixed parameter (7.43)\cite{be_table_2010}  \\
Fe$_{Cont}$ & Total number of $^{55}$Fe events (counts) \\
R$_{Fe}$ & Ratio of K$_{\alpha}$ to K$_{\beta}$ for  $^{55}$Fe, fixed parameter (7.35)\cite{be_table_2010} \\
$\mu_{3}$ & Mean Energy of $^{55}$Fe K$_{\alpha}$ X-ray, fixed parameter (5895~keV) \\
$\mu_{4}$ & Mean Energy of $^{55}$Fe K$_{\alpha}$ X-ray, fixed parameter (6512~keV) \\
$\sigma_{3}$ & Width of the $^{55}$Fe K$_{\beta}$ peak (keV) \\
$\mu_{Aug}$ & Shared Auger mean (keV)\\
$\sigma_{Aug}$ & Shared Auger Width (keV) \\
A$_{BKG}$& Flat background for anti-coincidence data (counts per bin)\\
C$_{BKG}$& Flat background for coincidence data (counts per bin)\\
$\delta$ & Fraction of total events that are Augers \\
$\alpha_T$ & Total Internal Conversion Coefficient (From:~\cite{band_diracfock_2002} and~\cite{kibedi_evaluation_2008})\\
$\alpha_K$ & Internal Conversion Coefficient from k-shell (From:~\cite{band_diracfock_2002} and~\cite{kibedi_evaluation_2008})\\
$\eta_E$ & SDD X-ray/Auger efficiency, from Section~\ref{sec:FalseNegative}\\
$\varepsilon_e$ & MTAS conversion electron efficiency at 829 keV (from Geant 4 simulations).\\
P$_k$& Probability of k-shell electron caputre (Table of Radio Nuclides) \\
w$_k$& K-shell fluorescence yield for \Mn\ (Table of Radio Nuclides) \\
$B_m T$ & MTAS background rate multiplied by true coincidence window,from ~\ref{App:BmT} \\
$T$ & True coincidence window, from~\ref{subsec:SDD_Efficiency} \\
A & Activity of the source, from~\ref{subsec:Activity}   \\\hline




\end{tabular}
\caption[Simultaneous Fit Parameters]{\label{tab:Par_Def}Definition of the parameters involved in the fit defined in Equations~\ref{Eqn:Anti_Fit} and~\ref{Eqn:Coinc_Fit}.}
\end{table*}


\begin{table*}[ht]
\centering
\begin{tabular}{cl}\hline
Parameter & Value  \\\hline
$\nu$ & 1367464 $\pm$ 1321 \\
$\chi^2$/D.O.F & 173/512 = 3.38 \\
$\varepsilon_{\gamma}$ & 0.9778(1) \\
$\mu_{1}$ & 5.411~keV, fixed parameter \\
$\sigma_{1}$ & 0.08373(7) \\
$\mu_{2}$ & 5.966~keV, fixed parameter \\
$\sigma_{2}$ & 0.0878(2) \\
R$_{Mn}$ & 7.43, fixed parameter\\
Fe$_{Cont}$ & 2362 $\pm$ 76 \\
R$_{Fe}$ & 7.35, fixed parameter\\
$\mu_{3}$ & 5.895~keV, fixed parameter\\
$\mu_{4}$ & 6512~keV, fixed parameter\\
$\sigma_{3}$ & 0.078 (6)\\
$\mu_{Aug}$ & 4.98(3) \\
$\sigma_{Aug}$ & 0.45(1) \\
A$_{BKG}$& 4.22 (23)\\
C$_{BKG}$& 4.87 (27)\\
$\delta$ & 0.0368(12)  \\
$\alpha_t$ & 0.000275(4), fixed parameter \\
$\alpha_k$ & 0.000249(4), fixed parameter\\
$\eta_E$ & 0.259(39), fixed parameter\\
$\varepsilon_e$ & 0.026893(164), fixed parameter\\
P$_k$& 0.8896 (17), fixed parameter \\
w$_k$& 0.289(5), fixed parameter  \\
$B_m T$ & 0.0125(1), fixed parameter\\
$T$ & 0.000004735, fixed parameter\\
A & 14.41 $\pm$ 2.98, fixed parameter\\\hline

\end{tabular}
\caption[Simultaneous Fit Parameters values]{\label{tab:Par_Val}Values of the parameters involved in the fit defined in Equations~\ref{Eqn:Anti_Fit} and~\ref{Eqn:Coinc_Fit}.}
\end{table*}


\newpage
\subsection{No Conversion Electrons Approximation}\label{subsec:No_Conversion_Electrons}

To understand the physical significance of $\Sigma$ and $\Sigma^*$ (Eqn.~\ref{Eqn:Sigma} and~\ref{Eqn:Sigma_Star}) we make the assumption that internal conversion is not possible (i.e. $\alpha_T$ = $\alpha_K$ = 0). Then Eqn.~\ref{Eqn:Sigma} and~\ref{Eqn:Sigma_Star} reduce to:

\begin{equation}\label{Eqn:Sigma_Star_No_Con}
 \Sigma^* =  \nu
        \left(\varepsilon^\prime_\gamma \right)
\end{equation}
and
\begin{equation}\label{Eqn:Sigma_No_Con}
\Sigma = \nu \left(1 - \varepsilon^\prime_\gamma \right).
\end{equation}

Here we see that $\Sigma$ and $\Sigma^*$ are just fractions of the total X-ray signal events but separated into anti-coincidence or coincidence grouping. The separation is performed by the $(\varepsilon^\prime_{\gamma})$ and $(1-\varepsilon^\prime_{\gamma}$) terms. The additional terms in Eqn.~\ref{Eqn:Sigma} and~\ref{Eqn:Sigma_Star} deal with the different cases that arise from potentially having a conversion electron form. Those cases are discussed in Liliannas document: \emph{Effect of SDD Tagging-Efficiency of Conversion Electrons in KDK Analysis}. 


\subsection{Systematic Uncertainties}\label{subsec:Syst_uncertainty}
Parameters  ($\alpha_t$, $\alpha_k$, $\eta_E$, $\varepsilon_e $, P$_k$, w$_k$, $B_m T$, A)  are taken from the literature ($\alpha_t$, $\alpha_k$, $\eta_E$, P$_k$,w$_k$), measurements ($\eta_E$, $B_m T$, A) or simulations ($\varepsilon_e $), see Tab.~\ref{tab:Par_Def}. Their contributions to systematic uncertainties are evaluated using the shift method defined in~\cite{heinrich_systematic_2007}. 
Firstly, the fit is performed at the nominal parameter values shown in Table~\ref{tab:Par_Val} which determines the nominal efficiency. Then a nuisance parameter is shifted up by 1 std. and the fit is performed again. The new efficiency is subtracted from the nominal value giving the upper systematic error for this nuisance parameter. This is repeated for all nuisance parameters and the results are added in quadrature, giving the total upper systematic. The process is repeated but lowering the nuisance parameter by 1 std. instead, thus giving the lower systematic uncertainty. For example, the \Mn, 2$\mu s$ Total data set gave a nominal efficiency of 0.97814 $\pm$ 0.00013 (Stat), with the shift method giving an upper systematic uncertainty of +0.00008 and a lower systematic uncertainty of  -0.00006. These systematic uncertainties are approximately a factor of 2 smaller than statistical uncertainty, so we only report the statistical uncertainty (rounded down) which can be seen in Table~\ref{tab:Modular_Efficiency}. Two things are important to note here, firstly the shift method of evaluating the systematic uncertainty can only be used if the efficiency behaves approximately linear over the region the nuisance parameters have been varied. This is true in our case and has been proven. Secondly it is important to include the effect of the conversion electrons in the likelihood, without this effect the retrieved value of the efficiency would be approximately 0.05$\%$ lower which is on the order of magnitude of the precision we are looking for, see Section~\ref{App:Conversion_Electrons}. 



\begin{table*}[ht]
\centering
\begin{tabular}{lccc}\hline
Coincidence Window & 1 $\mu s$ & 2 $\mu s$ & 4 $\mu s$\\\hline
Auger Not Included (Expo BKG) & 0.977784 $\pm$
0.000134 & 0.978146
$\pm$ 0.000129 & 0.978421$\pm$
0.000131 \\
Auger Included (Expo. BKG) & 0.977705 $\pm$
0.000126 & 0.978071
$\pm$ 0.000125 & 0.978348 $\pm$
0.000127\\
Gauss Auger Model & 0.977697 $\pm$ 0.000134 & 0.978063 $\pm$ 0.000131 & 0.978340 $\pm$ 0.00013 \\
No Conversion Electrons & 0.977023 $\pm$ 0.000131 & 0.977267 $\pm$ 0.000134 &0.977292 $\pm$ 0.000134\\
MTAS BKG Correction &0.977511 $\pm$ 0.000135 & 0.977758 $\pm$ 0.000134 & 0.977788 $\pm$ 0.000134\\\hline


\end{tabular}
\caption[Simultaneous Fit Parameters values]{\label{tab:W_WO_Auger}Difference in the measurement of $\varepsilon_\gamma$ when including/not including the Augers as contributors to the signal likelihood, when modelling the Auger as a gaussian or as an exponential, when not including the conversion electron correction and when including the MTAS BKG coincidence correction.}
\end{table*}

\newpage

\subsection{Approximation of the activity of the Mn source}\label{subsec:Activity}

We can make an approximation of the activity from Fig.~\ref{Fig:X_Ray_Cut_Mn54_Mn54_Gamma_Convolution.eps}. In that figure the area under the black curve (x =1327345(1175) counts) can be represented by:

\begin{equation}\label{Eqn:Activity}
    x = A T_{Run}~I_{EC^*}~\varepsilon_\gamma~\eta_E.
\end{equation}

Where A is the activity (counts/s), $T_{run}$ is the run length ( $T_{run}$ = 375813 s), \BRECStar\ is the excited state branching ratio, $\varepsilon_\gamma$ is the gamma tagging efficiency ( $\varepsilon_\gamma$ = 0.98(1)) and $\eta_E$ ( $\eta_E$ = 0.25(5)) is the SDD tagging efficiency (X-ray or Auger) in a specific energy region. We can rearrange Eqn.~\ref{Eqn:Activity} and set \BRECStar = 1.0 to get


\begin{equation}\label{Eqn:Activity_2}
    A = \frac{x}{T \varepsilon_\gamma \eta_E} = 14.41 \mbox{ /s}
\end{equation}
and the uncertainty, 
\begin{equation}\label{Eqn:Activity Error}
    \sigma_A= \sqrt{\left(\frac{1}{T \varepsilon_\gamma \eta_E}\right)^2 (\sigma_x^2)+\left(\frac{x}{T \varepsilon_\gamma^2 \eta_E}\right)^2 (\sigma_\varepsilon^2)+\left(\frac{x}{T \varepsilon_\gamma \eta_E^2}\right)^2 (\sigma_\eta^2)} = 2.98 counts/s.
\end{equation}

This method calculates an activity of 14.41 $\pm$ 2.98 counts/s. The approximation of the input parameters is valid due to the small overall contribution of the activity in Eqn.~\ref{Eqn:epsilon_prime}.


